Properties of pseudoscalar flavour-singlet mesons from 2+1+1 twisted mass lattice QCD

We study properties of pseudoscalar flavour-singlet mesons from Wilson twisted mass lattice QCD with Nf=2+1+1 dynamical quark flavors. Results for masses are presented at three values of the lattice spacing and light quark masses corresponding to values of the pion mass from 230 MeV to 500 MeV. We briefly discuss scaling effects and the light and strange quark mass dependence of the eta mass. In addition we present an exploratory study using Osterwalder-Seiler type strange and charm valence quarks. This approach avoids some of the complications of the twisted mass heavy doublet. We present first results for matching valence and unitary actions and a comparison of statistical uncertainties.

==> plots/B85/massDep.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
  \setlength{\unitlength}{0.0500bp}%
  \begin{picture}(6480.00,5040.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(1078,704){\makebox(0,0)[r]{\strut{} 1}}%
      \put(1078,1286){\makebox(0,0)[r]{\strut{} 1.5}}%
      \put(1078,1867){\makebox(0,0)[r]{\strut{} 2}}%
      \put(1078,2449){\makebox(0,0)[r]{\strut{} 2.5}}%
      \put(1078,3030){\makebox(0,0)[r]{\strut{} 3}}%
      \put(1078,3612){\makebox(0,0)[r]{\strut{} 3.5}}%
      \put(1078,4193){\makebox(0,0)[r]{\strut{} 4}}%
      \put(1078,4775){\makebox(0,0)[r]{\strut{} 4.5}}%
      \put(1210,484){\makebox(0,0){\strut{} 0.05}}%
      \put(1916,484){\makebox(0,0){\strut{} 0.06}}%
      \put(2621,484){\makebox(0,0){\strut{} 0.07}}%
      \put(3327,484){\makebox(0,0){\strut{} 0.08}}%
      \put(4032,484){\makebox(0,0){\strut{} 0.09}}%
      \put(4738,484){\makebox(0,0){\strut{} 0.1}}%
      \put(5443,484){\makebox(0,0){\strut{} 0.11}}%
      \put(6149,484){\makebox(0,0){\strut{} 0.12}}%
      \put(308,2739){\rotatebox{-270}{\makebox(0,0){\strut{}$m_\mathrm{eff}\cdot r_0$}}}%
      \put(3679,154){\makebox(0,0){\strut{}$\mu_s\cdot r_0$}}%
      \put(1296,4535){\makebox(0,0)[l]{\strut{}B85.24 ensemble}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(5162,4602){\makebox(0,0)[r]{\strut{}$\eta$}}%
      \csname LTb\endcsname%
      \put(5162,4382){\makebox(0,0)[r]{\strut{}unitary $\eta$}}%
      \csname LTb\endcsname%
      \put(5162,4162){\makebox(0,0)[r]{\strut{}$\eta'$}}%
      \csname LTb\endcsname%
      \put(5162,3942){\makebox(0,0)[r]{\strut{}unitary $\eta'$}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{massDep}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> plots/D45/d45evV.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
  \setlength{\unitlength}{0.0500bp}%
  \begin{picture}(7200.00,5760.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(1078,986){\makebox(0,0)[r]{\strut{} 0.4}}%
      \put(1078,1549){\makebox(0,0)[r]{\strut{} 0.6}}%
      \put(1078,2113){\makebox(0,0)[r]{\strut{} 0.8}}%
      \put(1078,2677){\makebox(0,0)[r]{\strut{} 1}}%
      \put(1078,3240){\makebox(0,0)[r]{\strut{} 1.2}}%
      \put(1078,3804){\makebox(0,0)[r]{\strut{} 1.4}}%
      \put(1078,4368){\makebox(0,0)[r]{\strut{} 1.6}}%
      \put(1078,4931){\makebox(0,0)[r]{\strut{} 1.8}}%
      \put(1078,5495){\makebox(0,0)[r]{\strut{} 2}}%
      \put(1210,484){\makebox(0,0){\strut{} 0}}%
      \put(2153,484){\makebox(0,0){\strut{} 5}}%
      \put(3096,484){\makebox(0,0){\strut{} 10}}%
      \put(4040,484){\makebox(0,0){\strut{} 15}}%
      \put(4983,484){\makebox(0,0){\strut{} 20}}%
      \put(5926,484){\makebox(0,0){\strut{} 25}}%
      \put(6869,484){\makebox(0,0){\strut{} 30}}%
      \put(308,3099){\rotatebox{-270}{\makebox(0,0){\strut{}$\delta \lambda_{OS}/\delta \lambda_{US}$}}}%
      \put(4039,154){\makebox(0,0){\strut{}$t/a$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(5882,5322){\makebox(0,0)[r]{\strut{}$\eta$}}%
      \csname LTb\endcsname%
      \put(5882,5102){\makebox(0,0)[r]{\strut{}$\eta'$}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{d45evV}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> plots/D45/d45massV.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
  \setlength{\unitlength}{0.0500bp}%
  \begin{picture}(7200.00,5760.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(1078,704){\makebox(0,0)[r]{\strut{} 0.2}}%
      \put(1078,1183){\makebox(0,0)[r]{\strut{} 0.3}}%
      \put(1078,1662){\makebox(0,0)[r]{\strut{} 0.4}}%
      \put(1078,2141){\makebox(0,0)[r]{\strut{} 0.5}}%
      \put(1078,2620){\makebox(0,0)[r]{\strut{} 0.6}}%
      \put(1078,3099){\makebox(0,0)[r]{\strut{} 0.7}}%
      \put(1078,3579){\makebox(0,0)[r]{\strut{} 0.8}}%
      \put(1078,4058){\makebox(0,0)[r]{\strut{} 0.9}}%
      \put(1078,4537){\makebox(0,0)[r]{\strut{} 1}}%
      \put(1078,5016){\makebox(0,0)[r]{\strut{} 1.1}}%
      \put(1078,5495){\makebox(0,0)[r]{\strut{} 1.2}}%
      \put(1210,484){\makebox(0,0){\strut{} 0}}%
      \put(2625,484){\makebox(0,0){\strut{} 5}}%
      \put(4040,484){\makebox(0,0){\strut{} 10}}%
      \put(5454,484){\makebox(0,0){\strut{} 15}}%
      \put(6869,484){\makebox(0,0){\strut{} 20}}%
      \put(308,3099){\rotatebox{-270}{\makebox(0,0){\strut{}$\delta m_{OS} / \delta m_{US}$}}}%
      \put(4039,154){\makebox(0,0){\strut{}t/a}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(5882,5322){\makebox(0,0)[r]{\strut{}$\eta$}}%
      \csname LTb\endcsname%
      \put(5882,5102){\makebox(0,0)[r]{\strut{}$\eta'$}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{d45massV}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> plots/D45/massDep.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
  \setlength{\unitlength}{0.0500bp}%
  \begin{picture}(6480.00,5040.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(1078,704){\makebox(0,0)[r]{\strut{} 1}}%
      \put(1078,1286){\makebox(0,0)[r]{\strut{} 1.5}}%
      \put(1078,1867){\makebox(0,0)[r]{\strut{} 2}}%
      \put(1078,2449){\makebox(0,0)[r]{\strut{} 2.5}}%
      \put(1078,3030){\makebox(0,0)[r]{\strut{} 3}}%
      \put(1078,3612){\makebox(0,0)[r]{\strut{} 3.5}}%
      \put(1078,4193){\makebox(0,0)[r]{\strut{} 4}}%
      \put(1078,4775){\makebox(0,0)[r]{\strut{} 4.5}}%
      \put(1210,484){\makebox(0,0){\strut{} 0.06}}%
      \put(1827,484){\makebox(0,0){\strut{} 0.07}}%
      \put(2445,484){\makebox(0,0){\strut{} 0.08}}%
      \put(3062,484){\makebox(0,0){\strut{} 0.09}}%
      \put(3679,484){\makebox(0,0){\strut{} 0.1}}%
      \put(4297,484){\makebox(0,0){\strut{} 0.11}}%
      \put(4914,484){\makebox(0,0){\strut{} 0.12}}%
      \put(5532,484){\makebox(0,0){\strut{} 0.13}}%
      \put(6149,484){\makebox(0,0){\strut{} 0.14}}%
      \put(308,2739){\rotatebox{-270}{\makebox(0,0){\strut{}$m_\mathrm{eff}\cdot r_0$}}}%
      \put(3679,154){\makebox(0,0){\strut{}$\mu_s\cdot r_0$}}%
      \put(1296,4535){\makebox(0,0)[l]{\strut{}D45.32sc ensemble}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(5162,4602){\makebox(0,0)[r]{\strut{}$\eta$}}%
      \csname LTb\endcsname%
      \put(5162,4382){\makebox(0,0)[r]{\strut{}unitary $\eta$}}%
      \csname LTb\endcsname%
      \put(5162,4162){\makebox(0,0)[r]{\strut{}$\eta'$}}%
      \csname LTb\endcsname%
      \put(5162,3942){\makebox(0,0)[r]{\strut{}unitary $\eta'$}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{massDep}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> tuning.tex <==
\section{Tunning of the heavy quark masses}
